SLAMBooster: An Application-aware Controller for Approximation in SLAM

Simultaneous Localization and Mapping (SLAM) is the problem of constructing a map of a mobile agent's environment while localizing the agent within the map. Dense SLAM algorithms perform reconstruction and localization at pixel granularity. These algorithms require a lot of computational power, which has hindered their use on low-power resource-constrained devices. Approximate computing can be used to speed up SLAM implementations as long as the approximations do not prevent the agent from navigating correctly through the environment. Previous studies of approximation in SLAM have assumed that the entire trajectory of the agent is known before the agent starts, and they have focused on offline controllers that set approximation knobs at the start of the trajectory. In practice, the trajectory is not known ahead of time, and allowing knob settings to change dynamically opens up more opportunities for reducing computation time and energy. We describe SLAMBooster, an application-aware, online control system for dense SLAM that adaptively controls approximation knobs during the motion of the agent. SLAMBooster is based on a control technique called proportional-integral-derivative (PID) controller but our experiments showed this application-agnostic controller led to an unacceptable reduction in localization accuracy. To address this problem, SLAMBooster also exploits domain knowledge for controlling approximation by performing smooth surface detection and pose correction. We implemented SLAMBooster in the open-source SLAMBench framework and evaluated it on several trajectories. Our experiments show that on the average, SLAMBooster reduces the computation time by 72% and energy consumption by 35% on an embedded platform, while maintaining the accuracy of localization within reasonable bounds. These improvements make it feasible to deploy SLAM on a wider range of devices.

==> sections/naive-pseudocode.tex <==
\begin{algorithm*}[t]
    \caption{Naive \name controller for \kfusion applied on each input frame Frame$_t$.}
    \label{alg:naive-heuristic}
    \begin{algorithmic}[1]
        \newcommand\letequal{\ensuremath{\gets}\xspace}
        %This one follows the logic in the code
        \State Frame$_t$ \letequal \texttt{\kfusion.acquisition}()
        \If {$t$ $\leq$ {\small BOOTSTRAP\_FRAMES}}
        \State Knob$_t$ \letequal Knob$_{t-1}$\label{alg:start}
        \State Frame$_t$ \letequal \texttt{\kfusion.preprocessing}(Frame$_t$, Knob$_t$)
        \State Pose$_t$ \letequal \texttt{\kfusion.tracking}(Frame$_t$, Knob$_t$)
        \State \texttt{\kfusion.integration}(Pose$_t$, Frame$_t$, Knob$_t$)
        \State \texttt{\kfusion.raycasting}(Pose$_t$, Knob$_t$)
        \State \texttt{\kfusion.rendering}(Pose$_t$, Knob$_t$)\label{alg:end}
        \State \textbf{continue}
        \EndIf
        \State
        \If{velocity\_trigger$_{t-1}$}\label{alg:vel-start}
        \State \algemph{Knob$_t$ \letequal Knob$_{t-1}$ - 1 \Comment{Increase precision}}
        \Else
        \State \algemph{Knob$_t$ \letequal Knob$_{t-1}$ + 1 \Comment{Increase approximation}}
        \EndIf\label{alg:vel-end}
        \State
        \State Frame$_t$ \letequal \texttt{\kfusion.preprocessing}(Frame$_t$, Knob$_t$)
        \State Pose$_t$ \letequal \texttt{\kfusion.tracking}(Frame$_t$, Knob$_t$)
        \State
        %\State \Comment{Compute velocity trigger for next frame}
        \State \algemph{V$_t$ \letequal Pose$_t$ - Pose$_{t-1}$\Comment{Compute velocity trigger for next frame}}\label{alg:comp-start}
        \State \algemph{velocity\_window \letequal velocity\_window ${\oplus}$ V$_t$}
        \State \algemph{V$_{avg}$ \letequal \texttt{sum}(velocity\_window) / WINDOW\_LEN}
        \State \algemph{velocity\_ascending\_trigger \letequal \texttt{ascending\_detection}(velocity\_window)}
        \State \algemph{velocity\_trigger$_t$ \letequal (V$_t$ > THRESHOLD) || (V$_{avg}$ > AVG\_THRESHOLD)}
        \State \algemph{\hspace{85pt}|| velocity\_ascending\_trigger}\label{alg:comp-end}
        \State
        \State \texttt{\kfusion.integration}(Pose$_t$, Frame$_t$, Knob$_t$)
        \State \texttt{\kfusion.raycasting}(Pose$_t$, Knob$_t$)
        \State \texttt{\kfusion.rendering}(Pose$_t$, Knob$_t$)
    \end{algorithmic}
    % \swarnendu{I am not sure how to color line 12, 14 and 16. So we may want to remove the highlights from the other lines.}
\end{algorithm*}


==> sections/opt-pseudocode.tex <==
\begin{algorithm*}[t]
	\caption{Online controller for \kfusion applied on each input Frame$_t$.}
	\label{alg:heuristic}
	\begin{algorithmic}[1]
		\newcommand\letequal{\ensuremath{\gets}\xspace}

		%This one follows the logic in the code
		\State Frame$_t$ \letequal \texttt{\kfusion.acquisition}()
		\If {$t$ $\leq$ {\small BOOTSTRAP\_FRAMES}}
		\State Knob$_t$ \letequal Knob$_{t-1}$
		\State Frame$_t$ \letequal \texttt{\kfusion.preprocessing}(Frame$_t$, Knob$_t$)
		\State Pose$_t$ \letequal \texttt{\kfusion.tracking}(Frame$_t$, Knob$_t$)
		\State \texttt{\kfusion.integration}(Pose$_t$, Frame$_t$, Knob$_t$)
		\State \texttt{\kfusion.raycasting}(Pose$_t$, Knob$_t$)
		\State \texttt{\kfusion.rendering}(Pose$_t$, Knob$_t$)
		\State \textbf{continue}
		\EndIf
		\State
		\State \algopt{feature\_trigger \letequal \texttt{FeatureExtraction}(Frame$_t$)\label{alg:features}}

		\If{velocity\_trigger$_{t-1}$ \textbf{or} \algopt{feature\_trigger}}\label{alg:vel-start-opt}
		\State Knob$_t$ \letequal Knob$_{t-1}$ - 1 \Comment{Increase precision}
		\Else
		\State Knob$_t$ \letequal Knob$_{t-1}$ + 1 \Comment{Increase approximation}
		\EndIf\label{alg:vel-end-opt}

		\State

		\State Frame$_t$ \letequal \texttt{\kfusion.preprocessing}(Frame$_t$, Knob$_t$)
		\State Pose$_t$ \letequal \texttt{\kfusion.tracking}(Frame$_t$, Knob$_t$)
		\State

        \State V$_t$ \letequal Pose$_t$ - Pose$_{t-1}$\Comment{Compute velocity trigger for next frame}\label{alg:exp-start}

		\If{V$_t$ > EXTRAPOLATE\_THRES}
		\State \algopt{Pose$_t$ \letequal T$_{t-1}$ * Pose$_{t-1}$}
		\State \algopt{T$_t$ \letequal T$_{t-1}$}
		\Else
		\State \algopt{T$_t$ \letequal Pose$_t$ * Pose$_{t-1}^{-1}$}
		\EndIf\label{alg:exp-end}
        \State

		% \Comment{Compute velocity trigger for next frame}
		\State velocity\_window \letequal velocity\_window ${\oplus}$ V$_t$
		\State V$_{avg}$ \letequal \texttt{sum}(velocity\_window) / WINDOW\_LEN
		\State velocity\_ascending\_trigger \letequal \texttt{ascending\_detection}(velocity\_window)
		\State velocity\_trigger$_t$ \letequal (V$_t$ > THRESHOLD) || (V$_{avg}$ > AVG\_THRESHOLD)\\
		\hspace{85pt}|| velocity\_ascending\_trigger || \algopt{(V$_t$ > EXTRAPOLATE\_THRES)}
		\State
		\State \texttt{\kfusion.integration}(Pose$_t$, Frame$_t$, Knob$_t$)
		\State \texttt{\kfusion.raycasting}(Pose$_t$, Knob$_t$)
		\State \texttt{\kfusion.rendering}(Pose$_t$, Knob$_t$)

	\end{algorithmic}
\end{algorithm*}


==> sections/tb_inputs.tex <==
\begin{table}[t]
    % \renewcommand{\baselinestretch}{1}\small\normalsize
    % \renewcommand{\arraystretch}{1.1}
    \renewcommand\sfsmaller{}
    \centering
    \begin{footnotesize}
        \begin{tabular}{l|rr}
                            & \textbf{Source}    & \textbf{\# frames} \\
            \midrule
            \bench{lr0}     & ICL-NUIM~\cite{iclnuim}  & 1510      \\
            \bench{lr1}     & ICL-NUIM~\cite{iclnuim}  & 967       \\
            \bench{lr2}     & ICL-NUIM~\cite{iclnuim}  & 882       \\
            %\bench{lr3}     & ICL-NUIM~\cite{iclnuim}  & 1242      \\
            \midrule
            \bench{ktcn0}  & Collected & 1550      \\
            \bench{ktcn1}  & Collected & 800       \\
            \bench{lab0}    & Collected & 800       \\
            \bench{lab1}    & Collected & 1250      \\
            \bench{lab2}    & Collected & 1250      \\
            \bench{lab3}    & Collected & 1250      \\
            \bench{mr0}     & Collected & 929       \\
            \bench{mr1}     & Collected & 1494      \\
            \bench{mr2}     & Collected & 1450      \\
            \bench{off0} & Collected & 750       \\
            \bench{off1} & Collected & 1050      \\
            \bench{off2} & Collected & 1200      \\
            \bench{pd0}     & Collected & 1600      \\
            \bench{pd1}     & Collected & 1500      \\
        \end{tabular}
    \end{footnotesize}
    \swarnendu{The second column is redundant given the caption we have now.}
    \caption{Input trajectories used in our evaluation. The first four trajectories are from the ICL-NUIM RGB-D dataset~\cite{iclnuim} and the rest have been collected in-house.}
    \label{tb:inputs}
\end{table}

==> sections/tb_results_momentum.tex <==
\begin{table*}[t]
  % \renewcommand{\baselinestretch}{1}\small\normalsize
  % \renewcommand{\arraystretch}{1.1}
  \renewcommand\sfsmaller{}
  \centering
  \newcommand{\n}{\ensuremath{n}\xspace}
  \newcommand{\f}{\ensuremath{\mathit{f}}\xspace}
  \renewcommand\k[1]{#1}
  % \newcommand\num[1]{#1~}
  \newcommand\num[1]{0.#1}
  \newcommand\snum[1]{0.0#1}
  \begin{footnotesize}
    \begin{tabular}{l|r|rrr|rrr}
      & & \multicolumn{3}{c|}{\textbf{Default \Kfusion}} & \multicolumn{3}{c}{\textbf{\name}} \\
      & \multirow{2}{*}{\textbf{\# frames}} & \textbf{\% frames} & {\bf Computation} & {\bf ATE} & \textbf{\% frames} & {\bf Computation} &  {\bf ATE} \\
      & & \textbf{tracked} & \textbf{time (s)} & \textbf{(cm)} & \textbf{tracked} & \textbf{time (s)} & \textbf{(cm)}\\
      \midrule
      \bench{lr0} & 1510 & 100 & 0.011 & 0.98 & 100 & 0.004 & 1.46 \\
      \bench{lr1} & 967 & 100 & 0.012 & 0.61 & 100 & 0.003 & 2.53 \\
      \bench{lr2} & 882 & 100 & 0.012 & 1.07 & 100 & 0.007 & 1.16 \\
      %\bench{lr3} & 1242 & 93 & 0.013 & 17.38 & 99.9 & 0.007 & 16.01 \\
      \midrule
      \bench{ktcn0} & 1550 & 100 & 0.012 & 1.04  & 100 & 0.004 & 1.28 \\
      \bench{ktcn1} & 800 & 100 & 0.012 & 2.70 & 100 & 0.006 & 1.12 \\
      \bench{lab0} & 800 & 100 & 0.012 & 0.73 & 100 & 0.005 & 4.23 \\
      \bench{lab1} & 1250 & 100 & 0.012 & 0.39 & 100 & 0.005 & 1.02 \\
      \bench{lab2} & 1250 & 100 & 0.011 & 2.94 & 99.6 & 0.004 & 2.17 \\
      \bench{lab3} & 1250 & 100 & 0.012 & 0.67 & 100 & 0.004 & 3.72 \\
      \bench{mr0} & 929 & 100 & 0.013 & 0.93 & 100 & 0.006 & 3.04 \\
      \bench{mr1} & 1494 & 100 & 0.013 & 2.33 & 100 & 0.007 & 3.47 \\
      \bench{mr2} & 1450 & 100 & 0.012 & 0.38 & 100 & 0.004 & 2.84 \\
      \bench{off0} & 750 & 100 & 0.011 & 0.16 & 100 & 0.006 & 1.01 \\
      \bench{off1} & 1050 & 100 & 0.013 & 0.77 & 100 & 0.007 & 0.77 \\
      \bench{off2} & 1200 & 100 & 0.012 & 0.45 & 100 & 0.005 & 1.07 \\
      \bench{pd0} & 1600 & 99.8 & 0.013 & 0.24 & 98.9 & 0.002 & 2.41 \\
      \bench{pd1} & 1500 & 100 & 0.012 & 0.61 & 100 & 0.004 & 3.44 \\
    \end{tabular}
  \end{footnotesize}
  \caption{Detailed results with input trajectories controlled using the \name control system on the Intel Xeon platform.
  % The first four trajectories are from the ICL-NUIM RGB-D dataset~\cite{iclnuim} and the rest have been collected in-house.
  }
  \label{tb:results-momentum}
\end{table*}

